MOT20: A benchmark for multi object tracking in crowded scenes

Standardized benchmarks are crucial for the majority of computer vision applications. Although leaderboards and ranking tables should not be over-claimed, benchmarks often provide the most objective measure of performance and are therefore important guides for research. The benchmark for Multiple Object Tracking, MOTChallenge, was launched with the goal to establish a standardized evaluation of multiple object tracking methods. The challenge focuses on multiple people tracking, since pedestrians are well studied in the tracking community, and precise tracking and detection has high practical relevance. Since the first release, MOT15, MOT16, and MOT17 have tremendously contributed to the community by introducing a clean dataset and precise framework to benchmark multi-object trackers. In this paper, we present our MOT20benchmark, consisting of 8 new sequences depicting very crowded challenging scenes. The benchmark was presented first at the 4thBMTT MOT Challenge Workshop at the Computer Vision and Pattern Recognition Conference (CVPR) 2019, and gives to chance to evaluate state-of-the-art methods for multiple object tracking when handling extremely crowded scenarios.

==> baseline.tex <==
\section{Baseline Methods}
\label{sec:baselines}
As a starting point for the benchmark, we are working on including a number of 
recent multi-target tracking approaches as baselines, which we will 
briefly outline for completeness but refer the reader to the respective 
publication for more details. Note that we have used the publicly 
available code and trained all of them in the same way
%\footnote{Except 
%for \Tracker{TBD}, which does not disclose any obvious free parameters.}
(\cf~\Sec~\ref{sec:training}). 
However, we explicitly state that the 
provided numbers may not represent the best possible performance for 
each method, as could be achieved by the authors themselves. 
Table~\ref{tab:results} lists current benchmark results for all 
baselines as well as for all anonymous entries at the time of 
writing of this manuscript.

%%%%%%%%%%%%%%%%%%%%%%%%
% RESULTS TABLE
%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[tb]
\begin {center}
\setlength{\tabcolsep}{0.15cm}
\begin{tabular}{l| rrrrrrrrrrrrr}
%\begin{tabular}{l| p{1cm} p{1.1cm} p{0.6cm}p{0.6cm}p{0.7cm}p{0.7cm}p{0.6cm}p{0.6cm}p{0.5cm}p{0.6cm}p{0.5cm}p{0.6cm}p{0.5cm}p{1.2cm}}
Method &  MOTA & MOTP & FAR & MT(\%) & ML(\%) & FP & FN & IDsw & rel.ID & FM & rel.FM & Hz & Ref.\\
\hline
%\Tracker{MotiCon} & 9.3 & 23.1 {\tiny $\pm$16.4} & 70.9 & 1.8 & 4.7 & 52.0 & 10404 & 35844 & 1018 & 24.4 & 1061 & 25.5 & 1.4 & \cite{lealcvpr2014} \\
%\Tracker{LP2D} & 8.3 & 19.8 {\tiny $\pm$14.2} & 71.2 & 2.0 & 6.7 & 41.2 & 11580 & 36045 & 1649 & 39.9 & 1712 & 41.4 & 112.1 & baseline\\
\Tracker{TBD} & 33.7 {\tiny $\pm$9.2} & 76.5 & 1.0 & 7.2 & 54.2 & 5,804 & 112,587 & 2,418 & 63.3 & 2,252 & 58.9 & 1.3 & \cite{Geiger:2014:PAMI}\\
\Tracker{CEM} & 33.2 {\tiny $\pm$7.9} & 75.8 & 1.2 & 7.8 & 54.4 & 6,837 & 114,322 & 642 & 17.2 & 731 & 19.6 &  0.3 & \cite{Milan:2014:PAMI}\\
%\Tracker{RMOT} & 10.6 & 18.6 {\tiny $\pm$17.5} & 69.6 & 2.2 & 5.3 & 53.3 & 12473 & 36835 & 684 & 17.1 & 1282 & 32.0 & 7.9 & \cite{yoonwacv2015}\\
\Tracker{DP\_NMS} & 32.2 {\tiny $\pm$9.8} & 76.4 & 0.2 & 5.4 & 62.1 & 1,123 & 121,579 & 972 & 29.2 & 944 & 28.3 & 212.6 & \cite{Pirsiavash:2011:CVPR} \\
\Tracker{SMOT} & 29.7 {\tiny $\pm$7.3} & 75.2 & 2.9 & 4.3 & 47.7 & 17,426 & 107,552 & 3,108 & 75.8 & 4,483 & 109.3 & 0.2 &  \cite{Dicle:2013:ICCV}\\
%\Tracker{TC\_ODAL} & 12.8 & 15.1 {\tiny $\pm$15.0} & 70.5 & 2.2 & 3.2 & 55.8 & 12970 & 38538 & 637 & 17.1 & 1716 & 46.0 & 1.7 & \cite{Bae:2014:CVPR}\\	
\Tracker{JPDA\_m} & 26.2 {\tiny $\pm$6.1} & 76.3 & 0.6 & 4.1 & 67.5 & 3,689 & 130,549 & 365 & 12.9 & 638 & 22.5 & 22.2 & \cite{Rezatofighi:2015:ICCV} \\

%
\end{tabular}
%%%%
\caption{Quantitative results of the baselines on MOT16.}
\label{tab:results}
\end{center}
\end{table*}

\subsection{Training and testing}
\label{sec:training}
Most of the available tracking approaches do not include a learning (or 
training) algorithm to determine the set of model parameters for a 
particular dataset. Therefore, we follow a simplistic search scheme for 
all baseline methods to find a good setting for our benchmark. To that 
end, we take the default parameter set $\parvec := 
\{\onepar_1,\ldots,\onepar_P\}$ as suggested by the authors, where $P$ is 
the number of free parameters for each method. We then perform 20 
independent runs 
on the training set with varying parameters. In each run, a parameter 
value $\onepar_i$ is uniformly sampled around its default value in the 
range $[\frac{1}{2}\onepar_i , 2 \onepar_i]$. Finally, the parameter set 
$\parvec^*$ that achieved the highest MOTA score across all 20 runs
(\cf~\Sec~\ref{sec:mota}) is taken as the optimal setting and run once 
on the test set. The optimal parameter set is stated in the description
entry for each baseline method on the benchmark website.

\subsection{\Tracker{DP\_NMS}: Network flow tracking}
\label{sec:DP_NMS}
Since its original publication \cite{Zhang:2008:CVPR}, a large number of 
methods that are based on the network flow formulation have appeared in 
the literature \cite{Pirsiavash:2011:CVPR, Butt:2013:CVPR, 
Liu:2013:CVPR, Wang:2014:CVPR, lealcvpr2012}. The basic idea is to model the tracking 
as a graph, where each node represents a detection and each edge 
represents a transition between two detections. Special source and sink 
nodes allow spawning and absorbing trajectories. A solution is obtained 
by finding the minimum cost flow in the graph. Multiple assignments and track 
splitting is prevented by introducing binary and linear constraints.

Here we use two solvers: (i) the successive shortest paths approach 
\cite{Pirsiavash:2011:CVPR} that employs dynamic programming with
non-maxima suppression, termed \Tracker{DP\_NMS}; (ii) a linear programming solver 
that appears as a baseline in \cite{lealcvpr2014}.
This solver uses the Gurobi Library \cite{gurobi}.

\subsection{\Tracker{CEM}: Continuous energy minimization}
\label{sec:CEM}
\Tracker{CEM} \cite{Milan:2014:PAMI} formulates the problem in terms of a 
high-dimensional continuous energy. Here, we use the basic approach 
\cite{Andriyenko:2011:CVPR} without explicit occlusion reasoning or 
appearance model. The target state $\mathbf{X}$ is represented by 
continuous $x,y$ coordinates in \emph{all} frames. The energy 
$E(\mathbf{X})$ is made up of several components, including a data term 
to keep the solution close to the observed data (detections), a dynamic 
model to smooth the trajectories, an exclusion term to avoid collisions, 
a persistence term to reduce track fragmentations, and a regularizer.
%
The resulting energy is highly non-convex and is minimized in an alternating
fashion using conjugate gradient descent and deterministic jump moves.

\subsection{\Tracker{SMOT}: Similar moving objects}
\label{sec:SMOT}
The Similar Multi-Object Tracking (\Tracker{SMOT}) approach 
\cite{Dicle:2013:ICCV} specifically targets situations where target 
appearance is ambiguous and rather concentrates on using the motion as a 
primary cue for data association. Tracklets with similar motion are linked
to longer trajectories using the generalized linear assignment (GLA) 
formulation. The motion similarity and the underlying dynamics of a 
tracklet are modeled as the order of a linear regressor approximating that
tracklet.



\subsection{\Tracker{TBD}: Tracking-by-detection}
\label{sec:TBD}
This two-stage tracking-by-detection (\Tracker{TBD}) approach 
\cite{Geiger:2014:PAMI, Zhang:2013:ICCV} is part of a larger traffic 
scene understanding framework and employs a rather simple data 
association technique. The first stage links overlapping detections
with similar appearance in successive frames into tracklets. The
second stage aims to bridge occlusions of up to 20 frames. Both stages
employ the Hungarian algorithm to optimally solve the matching problem.
Note that we did not re-train this baseline but rather used the original
implementation and parameters provided.

%
%\subsection{\Tracker{TC\_ODAL}: Tracklet confidence}
%\label{sec:TC_ODAL}
%
%Robust Online Multi-Object Tracking based on Tracklet Confidence and 
%Online Discriminative Appearance Learning, or \Tracker{TC\_ODAL} 
%\cite{Bae:2014:CVPR}, is the only online method among the baselines. It 
%proceeds in two stages. First, close detections are linked to form a set 
%of short, reliable tracklets. This so-called local association allows 
%one to progressively aggregate confident tracklets. In case of occlusions 
%or missed detections, the tracklet confidence value is decreased and a 
%global association is employed to bridge longer occlusion gaps. Both 
%association techniques are formulated as bipartite matching and tackled 
%with the Hungarian algorithm.
%
%Another prominent component of \Tracker{TC\_ODAL} is online appearance learning.
%To that end, positive samples are collected from tracklets with high
%confidence and incremental linear discriminant analysis (ILDA) is employed
%to update the appearance model in an online fashion.

\subsection{\Tracker{JPDA\_m}: Joint probabilistic data association using $m$-best solutions}
\label{sec:JPDAm}
Joint Probabilistic Data Association (JPDA)~\cite{Fortman:1980:MTT} is one of the oldest 
techniques for global data association. It first builds a joint hypothesis
probability that includes \emph{all} possible assignments, and then computes the
marginal probabilities for each target to be assigned to each measurement.
The state for each target is estimated in an online manner, typically using
one Kalman filter per target. While this approach is theoretically sound, it
is prohibitive in practice due to the exponential number of possible assignment
hypotheses to be considered. It has thus long been considered impractical for
computer vision applications, especially in crowded scenes.
Recently, an efficient approximation to JPDA was proposed~\cite{Rezatofighi:2015:ICCV}.
The main idea is to approximate the full joint probability distribution by $m$ strongest
hypotheses. It turns out that in practice, only around 100 most likely assignments
are sufficient to obtain the exact same solution as full JPDA.



==> biographies.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{laura.jpg}}]{Laura Leal-Taixe{\'e}}
received her Bachelor and Master degrees in Telecommunications Engineering from the Technical University of Catalonia (UPC), Barcelona. In 2008 she did her Master Thesis at Northeastern University, Boston, USA and in 2014 she received her PhD degree (Dr.-Ing.) from the Leibniz University Hannover, Germany. During her PhD she did a one-year visit at the Vision Lab at the University of Michigan, USA. She is currently a postdoctoral researcher at the Institute of Geodesy and Photogrammetry of ETH Zurich, Switzerland. 
Her research interests are multiple object tracking, with special focus on social motion models and global optimization methods, as well as scene understanding.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{anton.jpg}}]{Anton Milan}
(n{\'e} Andriyenko) received his Diplom degree in Computer Science (Dipl.-Inform.) from the University of Bonn in 2008. He has worked as a software developer in the computer graphics industry. Here received his PhD in 2013 from the Technical University Darmstadt, Germany, after which he visited the PRML group at the Hokkaido University in Japan. Since 2014, he is a post-doctoral researcher at the Australian Centre for Visual Technologies (ACVT) at the University of Adelaide. His research interests are energy-based optimization methods for real-world multiple people tracking scenarios.
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ian.jpg}}]{Ian Reid}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{stefan.jpg}}]{Stefan Roth}
received the Diplom degree in Computer Science and Engineering from the University of Mannheim, Germany in 2001. In 2003 he received the MSc degree in Computer Science from Brown University, and in 2007 the PhD degree in Computer Science from the same institution. Since 2007 he is an assistant professor of Computer Science at Technical University Darmstadt, Germany. His research interests include probabilistic and statistical approaches to image modeling, motion estimation,
human tracking, and object recognition. He received several awards, including an honorable mention for the Marr Prize at ICCV 2005 (with M. Black), the Olympus-Prize 2010 of the German Association for Pattern Recognition (DAGM) and the Heinz Maier-Leibnitz Prize 2012 of the German Research Foundation (DFG). He serves on the editorial board of the International Journal of Computer Vision (IJCV).
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{konrad.jpg}}]{Konrad Schindler}
received a Diplomingenieur (M.tech) degree in photogrammetry from Vienna University of Technology, Austria in 1999, and a PhD from Graz University of Technology, Austria, in 2003. He has worked as a photogrammetric engineer in the private industry, and held researcher positions in the Computer Graphics and Vision Department of Graz University of Technology, the Digital Perception Lab of Monash University, and the Computer Vision Lab of ETH Zurich. He became assistant professor of Image Understanding at TU Darmstadt in 2009, and since 2010 has been a tenured professor of Photogrammetry and Remote Sensing at ETH Zurich. His research interests lie in the field of computer vision, photogrammetry, and remote sensing, with a focus on image understanding and 3d reconstruction. He currently serves as head of the Institute of Geodesy and Photogrammetry, and as associate editor for the ISPRS Journal of Photogrammetry and Remote Sensing, and for the Image and Vision Computing Journal.
\end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> submission.tex <==
\section{Benchmark Submission}
\label{sec:benchmark-structure}
Our benchmark consists of the database and evaluation server on one hand, 
and the website as the user interface on the other. It is open to 
everyone who respects the submission policies (see next section). Before 
participating, every user is required to create an account providing
an institutional (as opposed to a generic) e-mail
address\footnote{For accountability and to prevent abuse by using several email accounts.}. 
After registering, the user can create a 
new tracker with a unique name and enter all additional details. It is 
mandatory to indicate
\begin{itemize}
\item the challenge or benchmark category in which the tracker will be 
participating,
%
\item the full name and a brief description of the method including the parameters used,

\item whether the method operates online or on a 
batch of frames and whether the source code is publicly available,

\item the \emph{total} runtime in seconds for computing the results on all 
sequences and the hardware used, and 
%
\item whether only the provided or also external training and detection 
data were used. 

%
\end{itemize}
%

%


After entering all details, it is possible to submit the results in 
the format described in \Sec~\ref{sec:data-format}. The tracking 
results will be automatically evaluated and appear on the user's profile. 
They will \emph{not} be displayed in the public ranking table. 
The user can then decide at any point in time to 
make the results public. Note that the results can be published anonymously,
\eg to enable a blind review process for a corresponding paper. In this case,
we ask to provide the venue and the paper ID or a similar unique reference.
We request that a proper reference to the method's description is added 
upon acceptance of the paper. In case of rejection, an anonymous entry may 
also be removed from the database. Anonymous entries will also be removed
after six months of inactivity.

The tracker's meta information such as description, or project page can be edited
at any time. Visual results of all public submissions, as well as annotations and
detections can be viewed on a dedicated 
visualization page.\footnote{\url{http://motchallenge.net/vis/}}



\subsection{Submission policy}
The main goal of this benchmark is to provide a platform that allows for 
an objective performance comparison of multiple target tracking 
approaches on real-world data. Therefore, we introduce a few simple 
guidelines that must be followed by all participants.

{\bf Training.} Ground truth is only provided for the training sequences.
It is the participant's own responsibility to find the best setting
using \emph{only} the training data.
The use of additional training data must be indicated during submission and will
be visible in the public ranking table.
The use of ground truth labels on the test data is strictly forbidden. This or any other misuse
of the benchmark will lead to the deletion of the participant's account and their results.

{\bf Detections.} We also provide a unique set of detections 
(see \Sec \ref{sec:detections}) for each sequence. We highly encourage all tracking-by-detection
algorithms to use the given detections. In case the user wants to present results with another set of
detections or is not using detections at all, this should be clearly stated during submission
and will also be displayed in the results table.
 
 {\bf Variations of the same tracker.} Each method corresponds to a single tracker created in the benchmark.
 Variations of the same method, \eg different features used, can only be evaluated on the training data.
 

{\bf Submission frequency.} Generally, we expect one single submission 
for every tracking approach. If for any reason, the user needs to 
re-compute and re-submit the results (\eg due to a bug discovered in the 
implementation), he/she may do so after a waiting period of 72 hours 
after the last submission. This policy should discourage the use of the
benchmark server for training and parameter tuning on the test data. The maximum number of
submissions per method is 4.
%
Under \emph{no} circumstances must anyone create a second account and 
attempt to re-submit in order to bypass the waiting period. This may lead
to a deletion of the account and excluding the user from participating
in the benchmark.

